Outlier-robust Kalman Filtering through Generalised Bayes

We derive a novel, provably robust, and closed-form Bayesian update rule for online filtering in state-space models in the presence of outliers and misspecified measurement models. Our method combines generalised Bayesian inference with filtering methods such as the extended and ensemble Kalman filter. We use the former to show robustness and the latter to ensure computational efficiency in the case of nonlinear models. Our method matches or outperforms other robust filtering methods (such as those based on variational Bayes) at a much lower computational cost. We show this empirically on a range of filtering problems with outlier measurements, such as object tracking, state estimation in high-dimensional chaotic systems, and online learning of neural networks.

==> packages.tex <==

\newcommand{\myeat}[1]{}
%http://www.stackprinter.com/export?service=tex.stackexchange&question=59702&printer=false&linktohome=true

%\usepackage[framemethod=TikZ]{mdframed}

% https://tex.stackexchange.com/questions/99049/latex-error-option-clash-for-package-xcolor-even-if-i-put-listings-before
%https://en.wikibooks.org/wiki/LaTeX/Colors
\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage[usenames]{color}

%\usepackage{float}
\usepackage{longtable}

\usepackage[toc,page]{appendix}

%\usepackage{tocloft}
%\advance\cftchapnumwidth 1cm
%https://tex.stackexchange.com/questions/436063/spacing-between-number-and-text-in-toc
%\advance\cftsecnumwidth 0.5em\relax


% https://mirror.las.iastate.edu/tex-archive/macros/latex/contrib/mathalpha/doc/mathalpha-doc.pdf
\usepackage{bm}
\usepackage{frcursive} 
\usepackage{xfrac}
\usepackage{mathrsfs}

\usepackage{fancyvrb} % https://tex.stackexchange.com/questions/122195/how-to-center-verbatim
\usepackage{xspace}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}

%https://tex.stackexchange.com/questions/58098/what-are-all-the-font-styles-i-can-use-in-math-mode
\usepackage[mathscr]{euscript}

\mathchardef\mhyphen="2D % Define a "math hyphen"
\mathchardef\mdash="2D % Define a "math hyphen"

%\usepackage{undertilde}
\usepackage{accents}


\usepackage[font={small,it}]{caption}
%\usepackage{subfigure}
\usepackage{subcaption} 
\usepackage{subfig}
%\usepackage{caption}
%\usepackage[font={small,it}]{subcaption} % https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Subfloats

%https://tex.stackexchange.com/questions/283324/different-font-sizes-for-figure-and-subfigure-captions/283327
%\captionsetup{font={footnotesize,it}}
%\captionsetup[sub]{font={footnotesize,it}}

%\usepackage[font={small,it}]{caption}
%\usepackage[font={footnotesize,it}]{caption}

\usepackage{url}
\usepackage{cancel} % \cancel for strikethrough
\usepackage{multirow}
\usepackage{multicol}




\usepackage{verbatim}
%\usepackage{comment} %http://www.ctan.org/tex-archive/macros/latex/contrib/comment/

% From https://media.nips.cc/Conferences/NIPS2017/Styles/nips_2017.tex
% https://tex.stackexchange.com/questions/406179/how-to-type-the-letter-%C5%81

\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% https://tex.stackexchange.com/questions/392208/command-k-unavailable-in-encoding-ot1-error-takes-me-to-line-which-doesnt-eve

%http://mirrors.ibiblio.org/CTAN/macros/latex/base/utf8ienc.pdf
\usepackage[utf8]{inputenc}
%\DeclareUnicodeCharacter{2010}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{2212}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{301}{-}% support older LaTeX versions
%\DeclareUnicodeCharacter{00B4}{\textasciiacute}
\DeclareUnicodeCharacter{00B4}{'}


\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography



%https://tex.stackexchange.com/questions/36660/only-authors-initials-in-bibtex-natbib-using-named-style

%http://mirrors.ibiblio.org/CTAN/macros/latex/exptl/biblatex/doc/biblatex.pdf
%  bibstyle=authortitle,
\usepackage[
  style=alphabetic,
  citestyle=alphabetic,
  natbib=true,
  backend=bibtex,
  maxcitenames=3,  mincitenames=1,
  maxbibnames=10,  minbibnames=1,
  firstinits=true,
  backref=false, 
  hyperref=true,
  doi=false,  isbn=false,  url=false,
  arxiv=abs
]{biblatex}

%https://tex.stackexchange.com/questions/36307/formatting-back-references-in-bibliography
\DefineBibliographyStrings{english}{%
  backrefpage = {page},% originally "cited on page"
  backrefpages = {pages},% originally "cited on pages"
}

\usepackage{xpatch}

\usepackage{booktabs}
\usepackage{comment}

\usepackage{paralist} % compactenunm, compactitem

\usepackage{tikz}
\usetikzlibrary{fit,arrows,calc,positioning,shadows.blur}

% https://www.overleaf.com/learn/how-to/Cross_referencing_with_the_xr_package_in_Overleaf
%https://tex.stackexchange.com/questions/14364/cross-referencing-between-different-files?noredirect=1&lq=1
%https://texfaq.org/FAQ-extref
\usepackage{xr}
%\usepackage{xr-hyper}
%\usepackage{zref-xr,zref-user}

%\externaldocument{app}


% From 	Mykel Kochenderfer 
\usepackage{mathtools}
\DeclarePairedDelimiter{\paren}{\lparen}{\rparen}
\DeclarePairedDelimiter{\brock}{\lbrack}{\rbrack}

\usepackage{enumitem}


%\usepackage{algorithm}
%\usepackage{algpseudocode}

% https://jdhao.github.io/2019/09/21/latex_algorithm_pseudo_code/

\usepackage[ruled,vlined,linesnumbered,algochapter]{algorithm2e}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage[noend]{algpseudocode}
%\usepackage{algorithmic}
\DontPrintSemicolon
\newcommand{\dontprintsemicolon}{}
% https://tex.stackexchange.com/questions/192435/adding-a-blank-line-in-algorithm2e

\usepackage{mdframed}
\usepackage{multicol}
\usepackage{rotating}
\usepackage{setspace}



\usepackage{blkarray}



%https://www.tug.org/FontCatalogue/newpx/
%https://wiki.carleton.edu/download/attachments/20155418/fontguide.pdf?version=1&modificationDate=1388599695000&api=v2
%\usepackage{newpxmath,newpxtext}

% https://tex.stackexchange.com/questions/514149/three-column-full-page-index-in-tufte-booktwoside-symmetric
%\usepackage[makeindex]{imakeidx}
\usepackage{imakeidx}
\usepackage[columns=3]{idxlayout}

% Hyperref needs to be last package
%https://tex.stackexchange.com/questions/326950/hyperref-conflicts-with-footnotea
%\usepackage[pagebackref=true,colorlinks=true,pdftex]{hyperref} % incompatible
%\usepackage[backref=true,colorlinks=true,pdftex]{hyperref} % incompatible

% https://tex.stackexchange.com/questions/35422/partition-numbering-and-pdf-bookmark-generation/35430#35430
\usepackage[bookmarksnumbered]{hyperref}

%\hypersetup{hidelinks,backref=true,pagebackref=true,hyperindex=true,hypertexnames=false,colorlinks=false,breaklinks=true,bookmarks=true,bookmarksopen=false,pdftitle={Title},pdfauthor={Author}}



\usepackage[capitalize]{cleveref}
%\usepackage{cleveref}
\Crefname{equation}{Equation}{Equations}
\crefname{equation}{Equation}{Equations}
\Crefname{section}{Section}{Sections}
\crefname{section}{Section}{Sections}
\Crefname{chapter}{Chapter}{Chapters}
\crefname{chapter}{Chapter}{Chapters}
\Crefname{figure}{Figure}{Figures}
\crefname{figure}{Figure}{Figures}
\Crefname{appsec}{Appendix}{Appendices}
\crefname{appsec}{Appendix}{Appendices}
%\usepackage[noabbrev,capitalize,nameinlink]{cleveref}


%https://robjhyndman.com/hyndsight/squeezing-space-with-latex/
%\usepackage{fontspec}
%setmonofont{DejaVu Sans Mono}[Scale=MatchLowercase]
%\setmainfont{DejaVu Sans}
%There is no ∇ (U+2207) in font ec-lmr10!

%http://www.gang.umass.edu/~franz/latexmanual.pdf


%https://image-color.com/color-picker#DA4F4F



\definecolor{cyan}{cmyk}{1,0,0,0.4}
\definecolor{magenta}{cmyk}{0,1,0,0.15}
\definecolor{yellow}{cmyk}{0,0,1,0}
\definecolor{black}{cmyk}{0,0,0,1}
\definecolor{orange}{cmyk}{0,0.5,1,0}
\definecolor{red}{cmyk}{0.00,0.92,0.92,0.06}
\definecolor{blue}{cmyk}{0.92,0.92,0.00,0.06}
\definecolor{green}{cmyk}{0.88,0.00,0.78,0.03}

\hypersetup{
    colorlinks,
    citecolor=magenta,
    linkcolor=magenta,
    urlcolor=cyan,
}

\usepackage{eqnalign}
\usepackage{version}

% Provide toggle to enable if..else conditions
\usepackage{etoolbox}

